Promise:Prompt-driven 3D Medical Image Segmentation Using Pretrained Image Foundation Models

To address prevalent issues in medical imaging, such as data acquisition challenges and label availability, transfer learning from natural to medical image domains serves as a viable strategy to produce reliable segmentation results. However, several existing barriers between domains need to be broken down, including addressing contrast discrepancies, managing anatomical variability, and adapting 2D pretrained models for 3D segmentation tasks. In this paper, we propose ProMISe,a prompt-driven 3D medical image segmentation model using only a single point prompt to leverage knowledge from a pretrained 2D image foundation model. In particular, we use the pretrained vision transformer from the Segment Anything Model (SAM) and integrate lightweight adapters to extract depth-related (3D) spatial context without updating the pretrained weights. For robust results, a hybrid network with complementary encoders is designed, and a boundary-aware loss is proposed to achieve precise boundaries. We evaluate our model on two public datasets for colon and pancreas tumor segmentations, respectively. Compared to the state-of-the-art segmentation methods with and without prompt engineering, our proposed method achieves superior performance. The code is publicly available at https://github.com/MedICL-VU/ProMISe.

==> text/_0-abstract_keywords.tex <==
\begin{abstract}


\\\\\\\\\\\\\\\\\\\\\\\
% THIS FILE DOESNT SEEM TO BE IN USE - ipek
\\\\\\\\\\\\\\\\\\\\\\\

To address prevalent issues in medical imaging, such as data acquisition challenges and label availability, transferring learning from natural to medical image domains serves as a viable strategy to produce reliable segmentation. However several existing barriers between domains need to be broken down include addressing contrast discrepancies, managing anatomical variability, and adapting 2D pretrained models for 3D segmentation tasks.
% However, several existing barriers between domains need to be broken down: (1) notable discrepancy in contrast, (2) complex anatomical variability in medical images, and (3) 2D pretrained image foundation models may struggle with 3D medical segmentation task.
In this paper, we propose Promise, a promptable model, for 3D medical image segmentation and utilize the knowledege from pretrained 2D image foundation model. Specifically, we use transformer image encoder from segment anything model and integrate lightweight adaptor to extract depth-related spatial features without updating the pretrained weights. Furthermore, we employ shallow networks for prompt generator and mask decoder tailored for volumetric medical segmentation. To achieve superior performance, hybrid network is designed with complementary encoders. We evaluate our model on two public datasets for colon and pancreas tumor segmentations, respectively. Compared to the state-of-the-art segmentation methods with and without prompt engineering, our proposed method achieves superior performance.
\end{abstract}


\begin{keywords}
Medical image segmentation, 3D adaptor, Transfer learning, Pretrained image foundation models, Segment anything model (SAM)
\end{keywords}


==> text/_2-related_works.tex <==
% \textbf{Adapting image foundation models.}


\\\\\\\\\\\\\\\\\\\\\\\
% THIS FILE DOESNT SEEM TO BE IN USE - ipek
\\\\\\\\\\\\\\\\\\\\\\\

Fully fine-tune image foundation models for a single task requires large amount computational resource and is not training-efficient. Instead, partially fine-tuning \cite{ma2023segment} or introducing and training new shallow layers, such as lightweight adapter \cite{pan2022st,chen2022adaptformer,yang2023aim,gong20233dsam,wu2023medical} and Low-Rank Adaptation (LoRA) module \cite{hu2021lora,zhang2023customized}, have demonstrated robust performance as parameter-efficient fine-tuning methods.
Recent works adapt SAM \cite{kirillov2023segment} for 3D medical data segmentation in a slice-wise manner, which discard important depth-wise information and may require additional effort to create prompt \cite{ma2023segment,zhang2023customized}. Leveraging insights from related works that demonstrate the effectiveness of utilizing adapters to adapt a pretrained model from 2D images to 3D videos \cite{pan2022st,yang2023aim}, this adaptation approach has subsequently been utilized in 3D medical image segmentation \cite{wu2023medical} with the use of adapters in the pretrained transformer block \cite{chen2022adaptformer}. Although it can segment 3D medical images, the image encoder still operates in a slice-wise manner with an additional branch for depth information. The weights for this branch that are replicated from the spatial branch demand more computational resources. In contrast, a holistic adaptation of SAM for 3D medical segmentation is proposed \cite{gong20233dsam} which avoids depth branch by including the adaptor with depth-wise convolution \cite{pan2022st}. However, a single adapter in each transformer block may not fully achieve accurate adaptation due to the notable discrepancies between nature and medical images. Moreover, their framework struggles to adequately capture the details of medical images, leading to suboptimal results, especially for tumor segmentation. Given current challenges and the critical importance of precise segmentation in medical applications, we are motivated to develop a robust solution that advances 3D medical image segmentation. 


